Search for a standard model-like Higgs boson in the mu+ mu- and e+ e- decay channels at the LHC

A search is presented for a standard model-like Higgs boson decaying to muon pair or electron pair final states based on proton-proton collisions recorded by the CMS experiment at the CERN LHC. The data correspond to integrated luminosities of 5.0 inverse femtobarns at a centre-of-mass energy of 7 TeV and 19.7 inverse femtobarns at 8 TeV for the muon search, and of 19.7 inverse femtobarns at 8 TeV for the electron search. Upper limits on the production cross section times branching fraction at the 95% confidence level are reported for Higgs boson masses in the range from 120 to 150 GeV. For a Higgs boson with a mass of 125 GeV decaying to muons, the observed (expected) upper limit on the production rate is found to be 7.4 (6.5 +2.8 -1.9) times the standard model value. This corresponds to an upper limit on the branching fraction of 0.0016. Similarly, for electrons, an upper limit of 0.0019 is placed on the branching fraction, which is about 3.7 E5 times the standard model value. These results, together with recent evidence of the 125 GeV boson coupling to tau-leptons with a larger branching fraction consistent with the standard model, confirm that the leptonic couplings of the new boson are not flavour-universal.

==> export/HIG-13-007-authorlist.tex <==
\textbf{Yerevan Physics Institute,  Yerevan,  Armenia}\\*[0pt]
V.~Khachatryan, A.M.~Sirunyan, A.~Tumasyan
\vskip\cmsinstskip
\textbf{Institut f\"{u}r Hochenergiephysik der OeAW,  Wien,  Austria}\\*[0pt]
W.~Adam, T.~Bergauer, M.~Dragicevic, J.~Er\"{o}, C.~Fabjan\cmsAuthorMark{1}, M.~Friedl, R.~Fr\"{u}hwirth\cmsAuthorMark{1}, V.M.~Ghete, C.~Hartl, N.~H\"{o}rmann, J.~Hrubec, M.~Jeitler\cmsAuthorMark{1}, W.~Kiesenhofer, V.~Kn\"{u}nz, M.~Krammer\cmsAuthorMark{1}, I.~Kr\"{a}tschmer, D.~Liko, I.~Mikulec, D.~Rabady\cmsAuthorMark{2}, B.~Rahbaran, H.~Rohringer, R.~Sch\"{o}fbeck, J.~Strauss, A.~Taurok, W.~Treberer-Treberspurg, W.~Waltenberger, C.-E.~Wulz\cmsAuthorMark{1}
\vskip\cmsinstskip
\textbf{National Centre for Particle and High Energy Physics,  Minsk,  Belarus}\\*[0pt]
V.~Mossolov, N.~Shumeiko, J.~Suarez Gonzalez
\vskip\cmsinstskip
\textbf{Universiteit Antwerpen,  Antwerpen,  Belgium}\\*[0pt]
S.~Alderweireldt, M.~Bansal, S.~Bansal, T.~Cornelis, E.A.~De Wolf, X.~Janssen, A.~Knutsson, S.~Luyckx, S.~Ochesanu, R.~Rougny, M.~Van De Klundert, H.~Van Haevermaet, P.~Van Mechelen, N.~Van Remortel, A.~Van Spilbeeck
\vskip\cmsinstskip
\textbf{Vrije Universiteit Brussel,  Brussel,  Belgium}\\*[0pt]
F.~Blekman, S.~Blyweert, J.~D'Hondt, N.~Daci, N.~Heracleous, J.~Keaveney, S.~Lowette, M.~Maes, A.~Olbrechts, Q.~Python, D.~Strom, S.~Tavernier, W.~Van Doninck, P.~Van Mulders, G.P.~Van Onsem, I.~Villella
\vskip\cmsinstskip
\textbf{Universit\'{e}~Libre de Bruxelles,  Bruxelles,  Belgium}\\*[0pt]
C.~Caillol, B.~Clerbaux, G.~De Lentdecker, D.~Dobur, L.~Favart, A.P.R.~Gay, A.~Grebenyuk, A.~L\'{e}onard, A.~Mohammadi, L.~Perni\`{e}\cmsAuthorMark{2}, T.~Reis, T.~Seva, L.~Thomas, C.~Vander Velde, P.~Vanlaer, J.~Wang, F.~Zenoni
\vskip\cmsinstskip
\textbf{Ghent University,  Ghent,  Belgium}\\*[0pt]
V.~Adler, K.~Beernaert, L.~Benucci, A.~Cimmino, S.~Costantini, S.~Crucy, S.~Dildick, A.~Fagot, G.~Garcia, J.~Mccartin, A.A.~Ocampo Rios, D.~Ryckbosch, S.~Salva Diblen, M.~Sigamani, N.~Strobbe, F.~Thyssen, M.~Tytgat, E.~Yazgan, N.~Zaganidis
\vskip\cmsinstskip
\textbf{Universit\'{e}~Catholique de Louvain,  Louvain-la-Neuve,  Belgium}\\*[0pt]
S.~Basegmez, C.~Beluffi\cmsAuthorMark{3}, G.~Bruno, R.~Castello, A.~Caudron, L.~Ceard, G.G.~Da Silveira, C.~Delaere, T.~du Pree, D.~Favart, L.~Forthomme, A.~Giammanco\cmsAuthorMark{4}, J.~Hollar, A.~Jafari, P.~Jez, M.~Komm, V.~Lemaitre, C.~Nuttens, D.~Pagano, L.~Perrini, A.~Pin, K.~Piotrzkowski, A.~Popov\cmsAuthorMark{5}, L.~Quertenmont, M.~Selvaggi, M.~Vidal Marono, J.M.~Vizan Garcia
\vskip\cmsinstskip
\textbf{Universit\'{e}~de Mons,  Mons,  Belgium}\\*[0pt]
N.~Beliy, T.~Caebergs, E.~Daubie, G.H.~Hammad
\vskip\cmsinstskip
\textbf{Centro Brasileiro de Pesquisas Fisicas,  Rio de Janeiro,  Brazil}\\*[0pt]
W.L.~Ald\'{a}~J\'{u}nior, G.A.~Alves, L.~Brito, M.~Correa Martins Junior, T.~Dos Reis Martins, C.~Mora Herrera, M.E.~Pol
\vskip\cmsinstskip
\textbf{Universidade do Estado do Rio de Janeiro,  Rio de Janeiro,  Brazil}\\*[0pt]
W.~Carvalho, J.~Chinellato\cmsAuthorMark{6}, A.~Cust\'{o}dio, E.M.~Da Costa, D.~De Jesus Damiao, C.~De Oliveira Martins, S.~Fonseca De Souza, H.~Malbouisson, D.~Matos Figueiredo, L.~Mundim, H.~Nogima, W.L.~Prado Da Silva, J.~Santaolalla, A.~Santoro, A.~Sznajder, E.J.~Tonelli Manganote\cmsAuthorMark{6}, A.~Vilela Pereira
\vskip\cmsinstskip
\textbf{Universidade Estadual Paulista~$^{a}$, ~Universidade Federal do ABC~$^{b}$, ~S\~{a}o Paulo,  Brazil}\\*[0pt]
C.A.~Bernardes$^{b}$, S.~Dogra$^{a}$, T.R.~Fernandez Perez Tomei$^{a}$, E.M.~Gregores$^{b}$, P.G.~Mercadante$^{b}$, S.F.~Novaes$^{a}$, Sandra S.~Padula$^{a}$
\vskip\cmsinstskip
\textbf{Institute for Nuclear Research and Nuclear Energy,  Sofia,  Bulgaria}\\*[0pt]
A.~Aleksandrov, V.~Genchev\cmsAuthorMark{2}, P.~Iaydjiev, A.~Marinov, S.~Piperov, M.~Rodozov, S.~Stoykova, G.~Sultanov, V.~Tcholakov, M.~Vutova
\vskip\cmsinstskip
\textbf{University of Sofia,  Sofia,  Bulgaria}\\*[0pt]
A.~Dimitrov, I.~Glushkov, R.~Hadjiiska, V.~Kozhuharov, L.~Litov, B.~Pavlov, P.~Petkov
\vskip\cmsinstskip
\textbf{Institute of High Energy Physics,  Beijing,  China}\\*[0pt]
J.G.~Bian, G.M.~Chen, H.S.~Chen, M.~Chen, R.~Du, C.H.~Jiang, R.~Plestina\cmsAuthorMark{7}, F.~Romeo, J.~Tao, Z.~Wang
\vskip\cmsinstskip
\textbf{State Key Laboratory of Nuclear Physics and Technology,  Peking University,  Beijing,  China}\\*[0pt]
C.~Asawatangtrakuldee, Y.~Ban, Q.~Li, S.~Liu, Y.~Mao, S.J.~Qian, D.~Wang, W.~Zou
\vskip\cmsinstskip
\textbf{Universidad de Los Andes,  Bogota,  Colombia}\\*[0pt]
C.~Avila, L.F.~Chaparro Sierra, C.~Florez, J.P.~Gomez, B.~Gomez Moreno, J.C.~Sanabria
\vskip\cmsinstskip
\textbf{University of Split,  Faculty of Electrical Engineering,  Mechanical Engineering and Naval Architecture,  Split,  Croatia}\\*[0pt]
N.~Godinovic, D.~Lelas, D.~Polic, I.~Puljak
\vskip\cmsinstskip
\textbf{University of Split,  Faculty of Science,  Split,  Croatia}\\*[0pt]
Z.~Antunovic, M.~Kovac
\vskip\cmsinstskip
\textbf{Institute Rudjer Boskovic,  Zagreb,  Croatia}\\*[0pt]
V.~Brigljevic, K.~Kadija, J.~Luetic, D.~Mekterovic, L.~Sudic
\vskip\cmsinstskip
\textbf{University of Cyprus,  Nicosia,  Cyprus}\\*[0pt]
A.~Attikis, G.~Mavromanolakis, J.~Mousa, C.~Nicolaou, F.~Ptochos, P.A.~Razis
\vskip\cmsinstskip
\textbf{Charles University,  Prague,  Czech Republic}\\*[0pt]
M.~Bodlak, M.~Finger, M.~Finger Jr.\cmsAuthorMark{8}
\vskip\cmsinstskip
\textbf{Academy of Scientific Research and Technology of the Arab Republic of Egypt,  Egyptian Network of High Energy Physics,  Cairo,  Egypt}\\*[0pt]
Y.~Assran\cmsAuthorMark{9}, A.~Ellithi Kamel\cmsAuthorMark{10}, M.A.~Mahmoud\cmsAuthorMark{11}, A.~Radi\cmsAuthorMark{12}$^{, }$\cmsAuthorMark{13}
\vskip\cmsinstskip
\textbf{National Institute of Chemical Physics and Biophysics,  Tallinn,  Estonia}\\*[0pt]
M.~Kadastik, M.~Murumaa, M.~Raidal, A.~Tiko
\vskip\cmsinstskip
\textbf{Department of Physics,  University of Helsinki,  Helsinki,  Finland}\\*[0pt]
P.~Eerola, G.~Fedi, M.~Voutilainen
\vskip\cmsinstskip
\textbf{Helsinki Institute of Physics,  Helsinki,  Finland}\\*[0pt]
J.~H\"{a}rk\"{o}nen, V.~Karim\"{a}ki, R.~Kinnunen, M.J.~Kortelainen, T.~Lamp\'{e}n, K.~Lassila-Perini, S.~Lehti, T.~Lind\'{e}n, P.~Luukka, T.~M\"{a}enp\"{a}\"{a}, T.~Peltola, E.~Tuominen, J.~Tuominiemi, E.~Tuovinen, L.~Wendland
\vskip\cmsinstskip
\textbf{Lappeenranta University of Technology,  Lappeenranta,  Finland}\\*[0pt]
J.~Talvitie, T.~Tuuva
\vskip\cmsinstskip
\textbf{DSM/IRFU,  CEA/Saclay,  Gif-sur-Yvette,  France}\\*[0pt]
M.~Besancon, F.~Couderc, M.~Dejardin, D.~Denegri, B.~Fabbro, J.L.~Faure, C.~Favaro, F.~Ferri, S.~Ganjour, A.~Givernaud, P.~Gras, G.~Hamel de Monchenault, P.~Jarry, E.~Locci, J.~Malcles, J.~Rander, A.~Rosowsky, M.~Titov
\vskip\cmsinstskip
\textbf{Laboratoire Leprince-Ringuet,  Ecole Polytechnique,  IN2P3-CNRS,  Palaiseau,  France}\\*[0pt]
S.~Baffioni, F.~Beaudette, P.~Busson, C.~Charlot, T.~Dahms, M.~Dalchenko, L.~Dobrzynski, N.~Filipovic, A.~Florent, R.~Granier de Cassagnac, L.~Mastrolorenzo, P.~Min\'{e}, C.~Mironov, I.N.~Naranjo, M.~Nguyen, C.~Ochando, P.~Paganini, S.~Regnard, R.~Salerno, J.B.~Sauvan, Y.~Sirois, C.~Veelken, Y.~Yilmaz, A.~Zabi
\vskip\cmsinstskip
\textbf{Institut Pluridisciplinaire Hubert Curien,  Universit\'{e}~de Strasbourg,  Universit\'{e}~de Haute Alsace Mulhouse,  CNRS/IN2P3,  Strasbourg,  France}\\*[0pt]
J.-L.~Agram\cmsAuthorMark{14}, J.~Andrea, A.~Aubin, D.~Bloch, J.-M.~Brom, E.C.~Chabert, C.~Collard, E.~Conte\cmsAuthorMark{14}, J.-C.~Fontaine\cmsAuthorMark{14}, D.~Gel\'{e}, U.~Goerlach, C.~Goetzmann, A.-C.~Le Bihan, P.~Van Hove
\vskip\cmsinstskip
\textbf{Centre de Calcul de l'Institut National de Physique Nucleaire et de Physique des Particules,  CNRS/IN2P3,  Villeurbanne,  France}\\*[0pt]
S.~Gadrat
\vskip\cmsinstskip
\textbf{Universit\'{e}~de Lyon,  Universit\'{e}~Claude Bernard Lyon 1, ~CNRS-IN2P3,  Institut de Physique Nucl\'{e}aire de Lyon,  Villeurbanne,  France}\\*[0pt]
S.~Beauceron, N.~Beaupere, G.~Boudoul\cmsAuthorMark{2}, E.~Bouvier, S.~Brochet, C.A.~Carrillo Montoya, J.~Chasserat, R.~Chierici, D.~Contardo\cmsAuthorMark{2}, P.~Depasse, H.~El Mamouni, J.~Fan, J.~Fay, S.~Gascon, M.~Gouzevitch, B.~Ille, T.~Kurca, M.~Lethuillier, L.~Mirabito, S.~Perries, J.D.~Ruiz Alvarez, D.~Sabes, L.~Sgandurra, V.~Sordini, M.~Vander Donckt, P.~Verdier, S.~Viret, H.~Xiao
\vskip\cmsinstskip
\textbf{Institute of High Energy Physics and Informatization,  Tbilisi State University,  Tbilisi,  Georgia}\\*[0pt]
Z.~Tsamalaidze\cmsAuthorMark{8}
\vskip\cmsinstskip
\textbf{RWTH Aachen University,  I.~Physikalisches Institut,  Aachen,  Germany}\\*[0pt]
C.~Autermann, S.~Beranek, M.~Bontenackels, M.~Edelhoff, L.~Feld, O.~Hindrichs, K.~Klein, A.~Ostapchuk, A.~Perieanu, F.~Raupach, J.~Sammet, S.~Schael, H.~Weber, B.~Wittmer, V.~Zhukov\cmsAuthorMark{5}
\vskip\cmsinstskip
\textbf{RWTH Aachen University,  III.~Physikalisches Institut A, ~Aachen,  Germany}\\*[0pt]
M.~Ata, M.~Brodski, E.~Dietz-Laursonn, D.~Duchardt, M.~Erdmann, R.~Fischer, A.~G\"{u}th, T.~Hebbeker, C.~Heidemann, K.~Hoepfner, D.~Klingebiel, S.~Knutzen, P.~Kreuzer, M.~Merschmeyer, A.~Meyer, P.~Millet, M.~Olschewski, K.~Padeken, P.~Papacz, H.~Reithler, S.A.~Schmitz, L.~Sonnenschein, D.~Teyssier, S.~Th\"{u}er, M.~Weber
\vskip\cmsinstskip
\textbf{RWTH Aachen University,  III.~Physikalisches Institut B, ~Aachen,  Germany}\\*[0pt]
V.~Cherepanov, Y.~Erdogan, G.~Fl\"{u}gge, H.~Geenen, M.~Geisler, W.~Haj Ahmad, A.~Heister, F.~Hoehle, B.~Kargoll, T.~Kress, Y.~Kuessel, A.~K\"{u}nsken, J.~Lingemann\cmsAuthorMark{2}, A.~Nowack, I.M.~Nugent, L.~Perchalla, O.~Pooth, A.~Stahl
\vskip\cmsinstskip
\textbf{Deutsches Elektronen-Synchrotron,  Hamburg,  Germany}\\*[0pt]
I.~Asin, N.~Bartosik, J.~Behr, W.~Behrenhoff, U.~Behrens, A.J.~Bell, M.~Bergholz\cmsAuthorMark{15}, A.~Bethani, K.~Borras, A.~Burgmeier, A.~Cakir, L.~Calligaris, A.~Campbell, S.~Choudhury, F.~Costanza, C.~Diez Pardos, S.~Dooling, T.~Dorland, G.~Eckerlin, D.~Eckstein, T.~Eichhorn, G.~Flucke, J.~Garay Garcia, A.~Geiser, P.~Gunnellini, J.~Hauk, M.~Hempel\cmsAuthorMark{15}, D.~Horton, H.~Jung, A.~Kalogeropoulos, M.~Kasemann, P.~Katsas, J.~Kieseler, C.~Kleinwort, D.~Kr\"{u}cker, W.~Lange, J.~Leonard, K.~Lipka, A.~Lobanov, W.~Lohmann\cmsAuthorMark{15}, B.~Lutz, R.~Mankel, I.~Marfin\cmsAuthorMark{15}, I.-A.~Melzer-Pellmann, A.B.~Meyer, G.~Mittag, J.~Mnich, A.~Mussgiller, S.~Naumann-Emme, A.~Nayak, O.~Novgorodova, E.~Ntomari, H.~Perrey, D.~Pitzl, R.~Placakyte, A.~Raspereza, P.M.~Ribeiro Cipriano, B.~Roland, E.~Ron, M.\"{O}.~Sahin, J.~Salfeld-Nebgen, P.~Saxena, R.~Schmidt\cmsAuthorMark{15}, T.~Schoerner-Sadenius, M.~Schr\"{o}der, C.~Seitz, S.~Spannagel, A.D.R.~Vargas Trevino, R.~Walsh, C.~Wissing
\vskip\cmsinstskip
\textbf{University of Hamburg,  Hamburg,  Germany}\\*[0pt]
M.~Aldaya Martin, V.~Blobel, M.~Centis Vignali, A.R.~Draeger, J.~Erfle, E.~Garutti, K.~Goebel, M.~G\"{o}rner, J.~Haller, M.~Hoffmann, R.S.~H\"{o}ing, H.~Kirschenmann, R.~Klanner, R.~Kogler, J.~Lange, T.~Lapsien, T.~Lenz, I.~Marchesini, J.~Ott, T.~Peiffer, N.~Pietsch, J.~Poehlsen, T.~Poehlsen, D.~Rathjens, C.~Sander, H.~Schettler, P.~Schleper, E.~Schlieckau, A.~Schmidt, M.~Seidel, V.~Sola, H.~Stadie, G.~Steinbr\"{u}ck, D.~Troendle, E.~Usai, L.~Vanelderen, A.~Vanhoefer
\vskip\cmsinstskip
\textbf{Institut f\"{u}r Experimentelle Kernphysik,  Karlsruhe,  Germany}\\*[0pt]
C.~Barth, C.~Baus, J.~Berger, C.~B\"{o}ser, E.~Butz, T.~Chwalek, W.~De Boer, A.~Descroix, A.~Dierlamm, M.~Feindt, F.~Frensch, M.~Giffels, F.~Hartmann\cmsAuthorMark{2}, T.~Hauth\cmsAuthorMark{2}, U.~Husemann, I.~Katkov\cmsAuthorMark{5}, A.~Kornmayer\cmsAuthorMark{2}, E.~Kuznetsova, P.~Lobelle Pardo, M.U.~Mozer, Th.~M\"{u}ller, A.~N\"{u}rnberg, G.~Quast, K.~Rabbertz, F.~Ratnikov, S.~R\"{o}cker, H.J.~Simonis, F.M.~Stober, R.~Ulrich, J.~Wagner-Kuhr, S.~Wayand, T.~Weiler, R.~Wolf
\vskip\cmsinstskip
\textbf{Institute of Nuclear and Particle Physics~(INPP), ~NCSR Demokritos,  Aghia Paraskevi,  Greece}\\*[0pt]
G.~Anagnostou, G.~Daskalakis, T.~Geralis, V.A.~Giakoumopoulou, A.~Kyriakis, D.~Loukas, A.~Markou, C.~Markou, A.~Psallidas, I.~Topsis-Giotis
\vskip\cmsinstskip
\textbf{University of Athens,  Athens,  Greece}\\*[0pt]
A.~Agapitos, S.~Kesisoglou, A.~Panagiotou, N.~Saoulidou, E.~Stiliaris
\vskip\cmsinstskip
\textbf{University of Io\'{a}nnina,  Io\'{a}nnina,  Greece}\\*[0pt]
X.~Aslanoglou, I.~Evangelou, G.~Flouris, C.~Foudas, P.~Kokkas, N.~Manthos, I.~Papadopoulos, E.~Paradas
\vskip\cmsinstskip
\textbf{Wigner Research Centre for Physics,  Budapest,  Hungary}\\*[0pt]
G.~Bencze, C.~Hajdu, P.~Hidas, D.~Horvath\cmsAuthorMark{16}, F.~Sikler, V.~Veszpremi, G.~Vesztergombi\cmsAuthorMark{17}, A.J.~Zsigmond
\vskip\cmsinstskip
\textbf{Institute of Nuclear Research ATOMKI,  Debrecen,  Hungary}\\*[0pt]
N.~Beni, S.~Czellar, J.~Karancsi\cmsAuthorMark{18}, J.~Molnar, J.~Palinkas, Z.~Szillasi
\vskip\cmsinstskip
\textbf{University of Debrecen,  Debrecen,  Hungary}\\*[0pt]
P.~Raics, Z.L.~Trocsanyi, B.~Ujvari
\vskip\cmsinstskip
\textbf{National Institute of Science Education and Research,  Bhubaneswar,  India}\\*[0pt]
S.K.~Swain
\vskip\cmsinstskip
\textbf{Panjab University,  Chandigarh,  India}\\*[0pt]
S.B.~Beri, V.~Bhatnagar, R.~Gupta, U.Bhawandeep, A.K.~Kalsi, M.~Kaur, R.~Kumar, M.~Mittal, N.~Nishu, J.B.~Singh
\vskip\cmsinstskip
\textbf{University of Delhi,  Delhi,  India}\\*[0pt]
Ashok Kumar, Arun Kumar, S.~Ahuja, A.~Bhardwaj, B.C.~Choudhary, A.~Kumar, S.~Malhotra, M.~Naimuddin, K.~Ranjan, V.~Sharma
\vskip\cmsinstskip
\textbf{Saha Institute of Nuclear Physics,  Kolkata,  India}\\*[0pt]
S.~Banerjee, S.~Bhattacharya, K.~Chatterjee, S.~Dutta, B.~Gomber, Sa.~Jain, Sh.~Jain, R.~Khurana, A.~Modak, S.~Mukherjee, D.~Roy, S.~Sarkar, M.~Sharan
\vskip\cmsinstskip
\textbf{Bhabha Atomic Research Centre,  Mumbai,  India}\\*[0pt]
A.~Abdulsalam, D.~Dutta, S.~Kailas, V.~Kumar, A.K.~Mohanty\cmsAuthorMark{2}, L.M.~Pant, P.~Shukla, A.~Topkar
\vskip\cmsinstskip
\textbf{Tata Institute of Fundamental Research,  Mumbai,  India}\\*[0pt]
T.~Aziz, S.~Banerjee, S.~Bhowmik\cmsAuthorMark{19}, R.M.~Chatterjee, R.K.~Dewanjee, S.~Dugad, S.~Ganguly, S.~Ghosh, M.~Guchait, A.~Gurtu\cmsAuthorMark{20}, G.~Kole, S.~Kumar, M.~Maity\cmsAuthorMark{19}, G.~Majumder, K.~Mazumdar, G.B.~Mohanty, B.~Parida, K.~Sudhakar, N.~Wickramage\cmsAuthorMark{21}
\vskip\cmsinstskip
\textbf{Institute for Research in Fundamental Sciences~(IPM), ~Tehran,  Iran}\\*[0pt]
H.~Bakhshiansohi, H.~Behnamian, S.M.~Etesami\cmsAuthorMark{22}, A.~Fahim\cmsAuthorMark{23}, R.~Goldouzian, M.~Khakzad, M.~Mohammadi Najafabadi, M.~Naseri, S.~Paktinat Mehdiabadi, F.~Rezaei Hosseinabadi, B.~Safarzadeh\cmsAuthorMark{24}, M.~Zeinali
\vskip\cmsinstskip
\textbf{University College Dublin,  Dublin,  Ireland}\\*[0pt]
M.~Felcini, M.~Grunewald
\vskip\cmsinstskip
\textbf{INFN Sezione di Bari~$^{a}$, Universit\`{a}~di Bari~$^{b}$, Politecnico di Bari~$^{c}$, ~Bari,  Italy}\\*[0pt]
M.~Abbrescia$^{a}$$^{, }$$^{b}$, L.~Barbone$^{a}$$^{, }$$^{b}$, C.~Calabria$^{a}$$^{, }$$^{b}$, S.S.~Chhibra$^{a}$$^{, }$$^{b}$, A.~Colaleo$^{a}$, D.~Creanza$^{a}$$^{, }$$^{c}$, N.~De Filippis$^{a}$$^{, }$$^{c}$, M.~De Palma$^{a}$$^{, }$$^{b}$, L.~Fiore$^{a}$, G.~Iaselli$^{a}$$^{, }$$^{c}$, G.~Maggi$^{a}$$^{, }$$^{c}$, M.~Maggi$^{a}$, S.~My$^{a}$$^{, }$$^{c}$, S.~Nuzzo$^{a}$$^{, }$$^{b}$, A.~Pompili$^{a}$$^{, }$$^{b}$, G.~Pugliese$^{a}$$^{, }$$^{c}$, R.~Radogna$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, G.~Selvaggi$^{a}$$^{, }$$^{b}$, L.~Silvestris$^{a}$$^{, }$\cmsAuthorMark{2}, R.~Venditti$^{a}$$^{, }$$^{b}$, G.~Zito$^{a}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Bologna~$^{a}$, Universit\`{a}~di Bologna~$^{b}$, ~Bologna,  Italy}\\*[0pt]
G.~Abbiendi$^{a}$, A.C.~Benvenuti$^{a}$, D.~Bonacorsi$^{a}$$^{, }$$^{b}$, S.~Braibant-Giacomelli$^{a}$$^{, }$$^{b}$, L.~Brigliadori$^{a}$$^{, }$$^{b}$, R.~Campanini$^{a}$$^{, }$$^{b}$, P.~Capiluppi$^{a}$$^{, }$$^{b}$, A.~Castro$^{a}$$^{, }$$^{b}$, F.R.~Cavallo$^{a}$, G.~Codispoti$^{a}$$^{, }$$^{b}$, M.~Cuffiani$^{a}$$^{, }$$^{b}$, G.M.~Dallavalle$^{a}$, F.~Fabbri$^{a}$, A.~Fanfani$^{a}$$^{, }$$^{b}$, D.~Fasanella$^{a}$$^{, }$$^{b}$, P.~Giacomelli$^{a}$, C.~Grandi$^{a}$, L.~Guiducci$^{a}$$^{, }$$^{b}$, S.~Marcellini$^{a}$, G.~Masetti$^{a}$, A.~Montanari$^{a}$, F.L.~Navarria$^{a}$$^{, }$$^{b}$, A.~Perrotta$^{a}$, F.~Primavera$^{a}$$^{, }$$^{b}$, A.M.~Rossi$^{a}$$^{, }$$^{b}$, T.~Rovelli$^{a}$$^{, }$$^{b}$, G.P.~Siroli$^{a}$$^{, }$$^{b}$, N.~Tosi$^{a}$$^{, }$$^{b}$, R.~Travaglini$^{a}$$^{, }$$^{b}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Catania~$^{a}$, Universit\`{a}~di Catania~$^{b}$, CSFNSM~$^{c}$, ~Catania,  Italy}\\*[0pt]
S.~Albergo$^{a}$$^{, }$$^{b}$, G.~Cappello$^{a}$, M.~Chiorboli$^{a}$$^{, }$$^{b}$, S.~Costa$^{a}$$^{, }$$^{b}$, F.~Giordano$^{a}$$^{, }$\cmsAuthorMark{2}, R.~Potenza$^{a}$$^{, }$$^{b}$, A.~Tricomi$^{a}$$^{, }$$^{b}$, C.~Tuve$^{a}$$^{, }$$^{b}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Firenze~$^{a}$, Universit\`{a}~di Firenze~$^{b}$, ~Firenze,  Italy}\\*[0pt]
G.~Barbagli$^{a}$, V.~Ciulli$^{a}$$^{, }$$^{b}$, C.~Civinini$^{a}$, R.~D'Alessandro$^{a}$$^{, }$$^{b}$, E.~Focardi$^{a}$$^{, }$$^{b}$, E.~Gallo$^{a}$, S.~Gonzi$^{a}$$^{, }$$^{b}$, V.~Gori$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, P.~Lenzi$^{a}$$^{, }$$^{b}$, M.~Meschini$^{a}$, S.~Paoletti$^{a}$, G.~Sguazzoni$^{a}$, A.~Tropiano$^{a}$$^{, }$$^{b}$
\vskip\cmsinstskip
\textbf{INFN Laboratori Nazionali di Frascati,  Frascati,  Italy}\\*[0pt]
L.~Benussi, S.~Bianco, F.~Fabbri, D.~Piccolo
\vskip\cmsinstskip
\textbf{INFN Sezione di Genova~$^{a}$, Universit\`{a}~di Genova~$^{b}$, ~Genova,  Italy}\\*[0pt]
R.~Ferretti$^{a}$$^{, }$$^{b}$, F.~Ferro$^{a}$, M.~Lo Vetere$^{a}$$^{, }$$^{b}$, E.~Robutti$^{a}$, S.~Tosi$^{a}$$^{, }$$^{b}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Milano-Bicocca~$^{a}$, Universit\`{a}~di Milano-Bicocca~$^{b}$, ~Milano,  Italy}\\*[0pt]
M.E.~Dinardo$^{a}$$^{, }$$^{b}$, S.~Fiorendi$^{a}$$^{, }$$^{b}$, S.~Gennai$^{a}$$^{, }$\cmsAuthorMark{2}, R.~Gerosa$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, A.~Ghezzi$^{a}$$^{, }$$^{b}$, P.~Govoni$^{a}$$^{, }$$^{b}$, M.T.~Lucchini$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, S.~Malvezzi$^{a}$, R.A.~Manzoni$^{a}$$^{, }$$^{b}$, A.~Martelli$^{a}$$^{, }$$^{b}$, B.~Marzocchi$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, D.~Menasce$^{a}$, L.~Moroni$^{a}$, M.~Paganoni$^{a}$$^{, }$$^{b}$, D.~Pedrini$^{a}$, S.~Ragazzi$^{a}$$^{, }$$^{b}$, N.~Redaelli$^{a}$, T.~Tabarelli de Fatis$^{a}$$^{, }$$^{b}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Napoli~$^{a}$, Universit\`{a}~di Napoli~'Federico II'~$^{b}$, Universit\`{a}~della Basilicata~(Potenza)~$^{c}$, Universit\`{a}~G.~Marconi~(Roma)~$^{d}$, ~Napoli,  Italy}\\*[0pt]
S.~Buontempo$^{a}$, N.~Cavallo$^{a}$$^{, }$$^{c}$, S.~Di Guida$^{a}$$^{, }$$^{d}$$^{, }$\cmsAuthorMark{2}, F.~Fabozzi$^{a}$$^{, }$$^{c}$, A.O.M.~Iorio$^{a}$$^{, }$$^{b}$, L.~Lista$^{a}$, S.~Meola$^{a}$$^{, }$$^{d}$$^{, }$\cmsAuthorMark{2}, M.~Merola$^{a}$, P.~Paolucci$^{a}$$^{, }$\cmsAuthorMark{2}
\vskip\cmsinstskip
\textbf{INFN Sezione di Padova~$^{a}$, Universit\`{a}~di Padova~$^{b}$, Universit\`{a}~di Trento~(Trento)~$^{c}$, ~Padova,  Italy}\\*[0pt]
P.~Azzi$^{a}$, N.~Bacchetta$^{a}$, D.~Bisello$^{a}$$^{, }$$^{b}$, A.~Branca$^{a}$$^{, }$$^{b}$, R.~Carlin$^{a}$$^{, }$$^{b}$, P.~Checchia$^{a}$, M.~Dall'Osso$^{a}$$^{, }$$^{b}$, T.~Dorigo$^{a}$, U.~Dosselli$^{a}$, M.~Galanti$^{a}$$^{, }$$^{b}$, F.~Gasparini$^{a}$$^{, }$$^{b}$, U.~Gasparini$^{a}$$^{, }$$^{b}$, P.~Giubilato$^{a}$$^{, }$$^{b}$, A.~Gozzelino$^{a}$, K.~Kanishchev$^{a}$$^{, }$$^{c}$, S.~Lacaprara$^{a}$, M.~Margoni$^{a}$$^{, }$$^{b}$, A.T.~Meneguzzo$^{a}$$^{, }$$^{b}$, J.~Pazzini$^{a}$$^{, }$$^{b}$, N.~Pozzobon$^{a}$$^{, }$$^{b}$, P.~Ronchese$^{a}$$^{, }$$^{b}$, F.~Simonetto$^{a}$$^{, }$$^{b}$, E.~Torassa$^{a}$, M.~Tosi$^{a}$$^{, }$$^{b}$, P.~Zotto$^{a}$$^{, }$$^{b}$, A.~Zucchetta$^{a}$$^{, }$$^{b}$, G.~Zumerle$^{a}$$^{, }$$^{b}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Pavia~$^{a}$, Universit\`{a}~di Pavia~$^{b}$, ~Pavia,  Italy}\\*[0pt]
M.~Gabusi$^{a}$$^{, }$$^{b}$, S.P.~Ratti$^{a}$$^{, }$$^{b}$, V.~Re$^{a}$, C.~Riccardi$^{a}$$^{, }$$^{b}$, P.~Salvini$^{a}$, P.~Vitulo$^{a}$$^{, }$$^{b}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Perugia~$^{a}$, Universit\`{a}~di Perugia~$^{b}$, ~Perugia,  Italy}\\*[0pt]
M.~Biasini$^{a}$$^{, }$$^{b}$, G.M.~Bilei$^{a}$, D.~Ciangottini$^{a}$$^{, }$$^{b}$, L.~Fan\`{o}$^{a}$$^{, }$$^{b}$, P.~Lariccia$^{a}$$^{, }$$^{b}$, G.~Mantovani$^{a}$$^{, }$$^{b}$, M.~Menichelli$^{a}$, A.~Saha$^{a}$, A.~Santocchia$^{a}$$^{, }$$^{b}$, A.~Spiezia$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}
\vskip\cmsinstskip
\textbf{INFN Sezione di Pisa~$^{a}$, Universit\`{a}~di Pisa~$^{b}$, Scuola Normale Superiore di Pisa~$^{c}$, ~Pisa,  Italy}\\*[0pt]
K.~Androsov$^{a}$$^{, }$\cmsAuthorMark{25}, P.~Azzurri$^{a}$, G.~Bagliesi$^{a}$, J.~Bernardini$^{a}$, T.~Boccali$^{a}$, G.~Broccolo$^{a}$$^{, }$$^{c}$, R.~Castaldi$^{a}$, M.A.~Ciocci$^{a}$$^{, }$\cmsAuthorMark{25}, R.~Dell'Orso$^{a}$, S.~Donato$^{a}$$^{, }$$^{c}$, F.~Fiori$^{a}$$^{, }$$^{c}$, L.~Fo\`{a}$^{a}$$^{, }$$^{c}$, A.~Giassi$^{a}$, M.T.~Grippo$^{a}$$^{, }$\cmsAuthorMark{25}, F.~Ligabue$^{a}$$^{, }$$^{c}$, T.~Lomtadze$^{a}$, L.~Martini$^{a}$$^{, }$$^{b}$, A.~Messineo$^{a}$$^{, }$$^{b}$, C.S.~Moon$^{a}$$^{, }$\cmsAuthorMark{26}, F.~Palla$^{a}$$^{, }$\cmsAuthorMark{2}, A.~Rizzi$^{a}$$^{, }$$^{b}$, A.~Savoy-Navarro$^{a}$$^{, }$\cmsAuthorMark{27}, A.T.~Serban$^{a}$, P.~Spagnolo$^{a}$, P.~Squillacioti$^{a}$$^{, }$\cmsAuthorMark{25}, R.~Tenchini$^{a}$, G.~Tonelli$^{a}$$^{, }$$^{b}$, A.~Venturi$^{a}$, P.G.~Verdini$^{a}$, C.~Vernieri$^{a}$$^{, }$$^{c}$$^{, }$\cmsAuthorMark{2}
\vskip\cmsinstskip
\textbf{INFN Sezione di Roma~$^{a}$, Universit\`{a}~di Roma~$^{b}$, ~Roma,  Italy}\\*[0pt]
L.~Barone$^{a}$$^{, }$$^{b}$, F.~Cavallari$^{a}$, G.~D'imperio$^{a}$$^{, }$$^{b}$, D.~Del Re$^{a}$$^{, }$$^{b}$, M.~Diemoz$^{a}$, M.~Grassi$^{a}$$^{, }$$^{b}$, C.~Jorda$^{a}$, E.~Longo$^{a}$$^{, }$$^{b}$, F.~Margaroli$^{a}$$^{, }$$^{b}$, P.~Meridiani$^{a}$, F.~Micheli$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, S.~Nourbakhsh$^{a}$$^{, }$$^{b}$, G.~Organtini$^{a}$$^{, }$$^{b}$, R.~Paramatti$^{a}$, S.~Rahatlou$^{a}$$^{, }$$^{b}$, C.~Rovelli$^{a}$, F.~Santanastasio$^{a}$$^{, }$$^{b}$, L.~Soffi$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, P.~Traczyk$^{a}$$^{, }$$^{b}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Torino~$^{a}$, Universit\`{a}~di Torino~$^{b}$, Universit\`{a}~del Piemonte Orientale~(Novara)~$^{c}$, ~Torino,  Italy}\\*[0pt]
N.~Amapane$^{a}$$^{, }$$^{b}$, R.~Arcidiacono$^{a}$$^{, }$$^{c}$, S.~Argiro$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, M.~Arneodo$^{a}$$^{, }$$^{c}$, R.~Bellan$^{a}$$^{, }$$^{b}$, C.~Biino$^{a}$, N.~Cartiglia$^{a}$, S.~Casasso$^{a}$$^{, }$$^{b}$$^{, }$\cmsAuthorMark{2}, M.~Costa$^{a}$$^{, }$$^{b}$, A.~Degano$^{a}$$^{, }$$^{b}$, N.~Demaria$^{a}$, L.~Finco$^{a}$$^{, }$$^{b}$, C.~Mariotti$^{a}$, S.~Maselli$^{a}$, E.~Migliore$^{a}$$^{, }$$^{b}$, V.~Monaco$^{a}$$^{, }$$^{b}$, M.~Musich$^{a}$, M.M.~Obertino$^{a}$$^{, }$$^{c}$$^{, }$\cmsAuthorMark{2}, G.~Ortona$^{a}$$^{, }$$^{b}$, L.~Pacher$^{a}$$^{, }$$^{b}$, N.~Pastrone$^{a}$, M.~Pelliccioni$^{a}$, G.L.~Pinna Angioni$^{a}$$^{, }$$^{b}$, A.~Potenza$^{a}$$^{, }$$^{b}$, A.~Romero$^{a}$$^{, }$$^{b}$, M.~Ruspa$^{a}$$^{, }$$^{c}$, R.~Sacchi$^{a}$$^{, }$$^{b}$, A.~Solano$^{a}$$^{, }$$^{b}$, A.~Staiano$^{a}$, U.~Tamponi$^{a}$
\vskip\cmsinstskip
\textbf{INFN Sezione di Trieste~$^{a}$, Universit\`{a}~di Trieste~$^{b}$, ~Trieste,  Italy}\\*[0pt]
S.~Belforte$^{a}$, V.~Candelise$^{a}$$^{, }$$^{b}$, M.~Casarsa$^{a}$, F.~Cossutti$^{a}$, G.~Della Ricca$^{a}$$^{, }$$^{b}$, B.~Gobbo$^{a}$, C.~La Licata$^{a}$$^{, }$$^{b}$, M.~Marone$^{a}$$^{, }$$^{b}$, A.~Schizzi$^{a}$$^{, }$$^{b}$, T.~Umer$^{a}$$^{, }$$^{b}$, A.~Zanetti$^{a}$
\vskip\cmsinstskip
\textbf{Kangwon National University,  Chunchon,  Korea}\\*[0pt]
S.~Chang, A.~Kropivnitskaya, S.K.~Nam
\vskip\cmsinstskip
\textbf{Kyungpook National University,  Daegu,  Korea}\\*[0pt]
D.H.~Kim, G.N.~Kim, M.S.~Kim, D.J.~Kong, S.~Lee, Y.D.~Oh, H.~Park, A.~Sakharov, D.C.~Son
\vskip\cmsinstskip
\textbf{Chonbuk National University,  Jeonju,  Korea}\\*[0pt]
T.J.~Kim
\vskip\cmsinstskip
\textbf{Chonnam National University,  Institute for Universe and Elementary Particles,  Kwangju,  Korea}\\*[0pt]
J.Y.~Kim, S.~Song
\vskip\cmsinstskip
\textbf{Korea University,  Seoul,  Korea}\\*[0pt]
S.~Choi, D.~Gyun, B.~Hong, M.~Jo, H.~Kim, Y.~Kim, B.~Lee, K.S.~Lee, S.K.~Park, Y.~Roh
\vskip\cmsinstskip
\textbf{University of Seoul,  Seoul,  Korea}\\*[0pt]
M.~Choi, J.H.~Kim, I.C.~Park, G.~Ryu, M.S.~Ryu
\vskip\cmsinstskip
\textbf{Sungkyunkwan University,  Suwon,  Korea}\\*[0pt]
Y.~Choi, Y.K.~Choi, J.~Goh, D.~Kim, E.~Kwon, J.~Lee, H.~Seo, I.~Yu
\vskip\cmsinstskip
\textbf{Vilnius University,  Vilnius,  Lithuania}\\*[0pt]
A.~Juodagalvis
\vskip\cmsinstskip
\textbf{National Centre for Particle Physics,  Universiti Malaya,  Kuala Lumpur,  Malaysia}\\*[0pt]
J.R.~Komaragiri, M.A.B.~Md Ali
\vskip\cmsinstskip
\textbf{Centro de Investigacion y~de Estudios Avanzados del IPN,  Mexico City,  Mexico}\\*[0pt]
H.~Castilla-Valdez, E.~De La Cruz-Burelo, I.~Heredia-de La Cruz\cmsAuthorMark{28}, A.~Hernandez-Almada, R.~Lopez-Fernandez, A.~Sanchez-Hernandez
\vskip\cmsinstskip
\textbf{Universidad Iberoamericana,  Mexico City,  Mexico}\\*[0pt]
S.~Carrillo Moreno, F.~Vazquez Valencia
\vskip\cmsinstskip
\textbf{Benemerita Universidad Autonoma de Puebla,  Puebla,  Mexico}\\*[0pt]
I.~Pedraza, H.A.~Salazar Ibarguen
\vskip\cmsinstskip
\textbf{Universidad Aut\'{o}noma de San Luis Potos\'{i}, ~San Luis Potos\'{i}, ~Mexico}\\*[0pt]
E.~Casimiro Linares, A.~Morelos Pineda
\vskip\cmsinstskip
\textbf{University of Auckland,  Auckland,  New Zealand}\\*[0pt]
D.~Krofcheck
\vskip\cmsinstskip
\textbf{University of Canterbury,  Christchurch,  New Zealand}\\*[0pt]
P.H.~Butler, S.~Reucroft
\vskip\cmsinstskip
\textbf{National Centre for Physics,  Quaid-I-Azam University,  Islamabad,  Pakistan}\\*[0pt]
A.~Ahmad, M.~Ahmad, Q.~Hassan, H.R.~Hoorani, S.~Khalid, W.A.~Khan, T.~Khurshid, M.A.~Shah, M.~Shoaib
\vskip\cmsinstskip
\textbf{National Centre for Nuclear Research,  Swierk,  Poland}\\*[0pt]
H.~Bialkowska, M.~Bluj, B.~Boimska, T.~Frueboes, M.~G\'{o}rski, M.~Kazana, K.~Nawrocki, K.~Romanowska-Rybinska, M.~Szleper, P.~Zalewski
\vskip\cmsinstskip
\textbf{Institute of Experimental Physics,  Faculty of Physics,  University of Warsaw,  Warsaw,  Poland}\\*[0pt]
G.~Brona, K.~Bunkowski, M.~Cwiok, W.~Dominik, K.~Doroba, A.~Kalinowski, M.~Konecki, J.~Krolikowski, M.~Misiura, M.~Olszewski, W.~Wolszczak
\vskip\cmsinstskip
\textbf{Laborat\'{o}rio de Instrumenta\c{c}\~{a}o e~F\'{i}sica Experimental de Part\'{i}culas,  Lisboa,  Portugal}\\*[0pt]
P.~Bargassa, C.~Beir\~{a}o Da Cruz E~Silva, P.~Faccioli, P.G.~Ferreira Parracho, M.~Gallinaro, L.~Lloret Iglesias, F.~Nguyen, J.~Rodrigues Antunes, J.~Seixas, J.~Varela, P.~Vischia
\vskip\cmsinstskip
\textbf{Joint Institute for Nuclear Research,  Dubna,  Russia}\\*[0pt]
P.~Bunin, I.~Golutvin, I.~Gorbunov, A.~Kamenev, V.~Karjavin, V.~Konoplyanikov, A.~Lanev, A.~Malakhov, V.~Matveev\cmsAuthorMark{29}, P.~Moisenz, V.~Palichik, V.~Perelygin, M.~Savina, S.~Shmatov, S.~Shulha, N.~Skatchkov, V.~Smirnov, A.~Zarubin
\vskip\cmsinstskip
\textbf{Petersburg Nuclear Physics Institute,  Gatchina~(St.~Petersburg), ~Russia}\\*[0pt]
V.~Golovtsov, Y.~Ivanov, V.~Kim\cmsAuthorMark{30}, P.~Levchenko, V.~Murzin, V.~Oreshkin, I.~Smirnov, V.~Sulimov, L.~Uvarov, S.~Vavilov, A.~Vorobyev, An.~Vorobyev
\vskip\cmsinstskip
\textbf{Institute for Nuclear Research,  Moscow,  Russia}\\*[0pt]
Yu.~Andreev, A.~Dermenev, S.~Gninenko, N.~Golubev, M.~Kirsanov, N.~Krasnikov, A.~Pashenkov, D.~Tlisov, A.~Toropin
\vskip\cmsinstskip
\textbf{Institute for Theoretical and Experimental Physics,  Moscow,  Russia}\\*[0pt]
V.~Epshteyn, V.~Gavrilov, N.~Lychkovskaya, V.~Popov, G.~Safronov, S.~Semenov, A.~Spiridonov, V.~Stolin, E.~Vlasov, A.~Zhokin
\vskip\cmsinstskip
\textbf{P.N.~Lebedev Physical Institute,  Moscow,  Russia}\\*[0pt]
V.~Andreev, M.~Azarkin, I.~Dremin, M.~Kirakosyan, A.~Leonidov, G.~Mesyats, S.V.~Rusakov, A.~Vinogradov
\vskip\cmsinstskip
\textbf{Skobeltsyn Institute of Nuclear Physics,  Lomonosov Moscow State University,  Moscow,  Russia}\\*[0pt]
A.~Belyaev, E.~Boos, V.~Bunichev, M.~Dubinin\cmsAuthorMark{31}, L.~Dudko, A.~Ershov, V.~Klyukhin, O.~Kodolova, I.~Lokhtin, S.~Obraztsov, M.~Perfilov, S.~Petrushanko, V.~Savrin
\vskip\cmsinstskip
\textbf{State Research Center of Russian Federation,  Institute for High Energy Physics,  Protvino,  Russia}\\*[0pt]
I.~Azhgirey, I.~Bayshev, S.~Bitioukov, V.~Kachanov, A.~Kalinin, D.~Konstantinov, V.~Krychkine, V.~Petrov, R.~Ryutin, A.~Sobol, L.~Tourtchanovitch, S.~Troshin, N.~Tyurin, A.~Uzunian, A.~Volkov
\vskip\cmsinstskip
\textbf{University of Belgrade,  Faculty of Physics and Vinca Institute of Nuclear Sciences,  Belgrade,  Serbia}\\*[0pt]
P.~Adzic\cmsAuthorMark{32}, M.~Ekmedzic, J.~Milosevic, V.~Rekovic
\vskip\cmsinstskip
\textbf{Centro de Investigaciones Energ\'{e}ticas Medioambientales y~Tecnol\'{o}gicas~(CIEMAT), ~Madrid,  Spain}\\*[0pt]
J.~Alcaraz Maestre, C.~Battilana, E.~Calvo, M.~Cerrada, M.~Chamizo Llatas, N.~Colino, B.~De La Cruz, A.~Delgado Peris, D.~Dom\'{i}nguez V\'{a}zquez, A.~Escalante Del Valle, C.~Fernandez Bedoya, J.P.~Fern\'{a}ndez Ramos, J.~Flix, M.C.~Fouz, P.~Garcia-Abia, O.~Gonzalez Lopez, S.~Goy Lopez, J.M.~Hernandez, M.I.~Josa, E.~Navarro De Martino, A.~P\'{e}rez-Calero Yzquierdo, J.~Puerta Pelayo, A.~Quintario Olmeda, I.~Redondo, L.~Romero, M.S.~Soares
\vskip\cmsinstskip
\textbf{Universidad Aut\'{o}noma de Madrid,  Madrid,  Spain}\\*[0pt]
C.~Albajar, J.F.~de Troc\'{o}niz, M.~Missiroli, D.~Moran
\vskip\cmsinstskip
\textbf{Universidad de Oviedo,  Oviedo,  Spain}\\*[0pt]
H.~Brun, J.~Cuevas, J.~Fernandez Menendez, S.~Folgueras, I.~Gonzalez Caballero
\vskip\cmsinstskip
\textbf{Instituto de F\'{i}sica de Cantabria~(IFCA), ~CSIC-Universidad de Cantabria,  Santander,  Spain}\\*[0pt]
J.A.~Brochero Cifuentes, I.J.~Cabrillo, A.~Calderon, J.~Duarte Campderros, M.~Fernandez, G.~Gomez, A.~Graziano, A.~Lopez Virto, J.~Marco, R.~Marco, C.~Martinez Rivero, F.~Matorras, F.J.~Munoz Sanchez, J.~Piedra Gomez, T.~Rodrigo, A.Y.~Rodr\'{i}guez-Marrero, A.~Ruiz-Jimeno, L.~Scodellaro, I.~Vila, R.~Vilar Cortabitarte
\vskip\cmsinstskip
\textbf{CERN,  European Organization for Nuclear Research,  Geneva,  Switzerland}\\*[0pt]
D.~Abbaneo, E.~Auffray, G.~Auzinger, M.~Bachtis, P.~Baillon, A.H.~Ball, D.~Barney, A.~Benaglia, J.~Bendavid, L.~Benhabib, J.F.~Benitez, C.~Bernet\cmsAuthorMark{7}, G.~Bianchi, P.~Bloch, A.~Bocci, A.~Bonato, O.~Bondu, C.~Botta, H.~Breuker, T.~Camporesi, G.~Cerminara, S.~Colafranceschi\cmsAuthorMark{33}, M.~D'Alfonso, D.~d'Enterria, A.~Dabrowski, A.~David, F.~De Guio, A.~De Roeck, S.~De Visscher, E.~Di Marco, M.~Dobson, M.~Dordevic, N.~Dupont-Sagorin, A.~Elliott-Peisert, J.~Eugster, G.~Franzoni, W.~Funk, D.~Gigi, K.~Gill, D.~Giordano, M.~Girone, F.~Glege, R.~Guida, S.~Gundacker, M.~Guthoff, J.~Hammer, M.~Hansen, P.~Harris, J.~Hegeman, V.~Innocente, P.~Janot, K.~Kousouris, K.~Krajczar, P.~Lecoq, C.~Louren\c{c}o, N.~Magini, L.~Malgeri, M.~Mannelli, J.~Marrouche, L.~Masetti, F.~Meijers, S.~Mersi, E.~Meschi, F.~Moortgat, S.~Morovic, M.~Mulders, P.~Musella, L.~Orsini, L.~Pape, E.~Perez, L.~Perrozzi, A.~Petrilli, G.~Petrucciani, A.~Pfeiffer, M.~Pierini, M.~Pimi\"{a}, D.~Piparo, M.~Plagge, A.~Racz, G.~Rolandi\cmsAuthorMark{34}, M.~Rovere, H.~Sakulin, C.~Sch\"{a}fer, C.~Schwick, A.~Sharma, P.~Siegrist, P.~Silva, M.~Simon, P.~Sphicas\cmsAuthorMark{35}, D.~Spiga, J.~Steggemann, B.~Stieger, M.~Stoye, Y.~Takahashi, D.~Treille, A.~Tsirou, G.I.~Veres\cmsAuthorMark{17}, N.~Wardle, H.K.~W\"{o}hri, H.~Wollny, W.D.~Zeuner
\vskip\cmsinstskip
\textbf{Paul Scherrer Institut,  Villigen,  Switzerland}\\*[0pt]
W.~Bertl, K.~Deiters, W.~Erdmann, R.~Horisberger, Q.~Ingram, H.C.~Kaestli, D.~Kotlinski, U.~Langenegger, D.~Renker, T.~Rohe
\vskip\cmsinstskip
\textbf{Institute for Particle Physics,  ETH Zurich,  Zurich,  Switzerland}\\*[0pt]
F.~Bachmair, L.~B\"{a}ni, L.~Bianchini, M.A.~Buchmann, B.~Casal, N.~Chanon, G.~Dissertori, M.~Dittmar, M.~Doneg\`{a}, M.~D\"{u}nser, P.~Eller, C.~Grab, D.~Hits, J.~Hoss, W.~Lustermann, B.~Mangano, A.C.~Marini, P.~Martinez Ruiz del Arbol, M.~Masciovecchio, D.~Meister, N.~Mohr, C.~N\"{a}geli\cmsAuthorMark{36}, F.~Nessi-Tedaldi, F.~Pandolfi, F.~Pauss, M.~Peruzzi, M.~Quittnat, L.~Rebane, M.~Rossini, A.~Starodumov\cmsAuthorMark{37}, M.~Takahashi, K.~Theofilatos, R.~Wallny, H.A.~Weber
\vskip\cmsinstskip
\textbf{Universit\"{a}t Z\"{u}rich,  Zurich,  Switzerland}\\*[0pt]
C.~Amsler\cmsAuthorMark{38}, M.F.~Canelli, V.~Chiochia, A.~De Cosa, A.~Hinzmann, T.~Hreus, B.~Kilminster, C.~Lange, B.~Millan Mejias, J.~Ngadiuba, P.~Robmann, F.J.~Ronga, S.~Taroni, M.~Verzetti, Y.~Yang
\vskip\cmsinstskip
\textbf{National Central University,  Chung-Li,  Taiwan}\\*[0pt]
M.~Cardaci, K.H.~Chen, C.~Ferro, C.M.~Kuo, W.~Lin, Y.J.~Lu, R.~Volpe, S.S.~Yu
\vskip\cmsinstskip
\textbf{National Taiwan University~(NTU), ~Taipei,  Taiwan}\\*[0pt]
P.~Chang, Y.H.~Chang, Y.W.~Chang, Y.~Chao, K.F.~Chen, P.H.~Chen, C.~Dietz, U.~Grundler, W.-S.~Hou, K.Y.~Kao, Y.J.~Lei, Y.F.~Liu, R.-S.~Lu, D.~Majumder, E.~Petrakou, Y.M.~Tzeng, R.~Wilken
\vskip\cmsinstskip
\textbf{Chulalongkorn University,  Faculty of Science,  Department of Physics,  Bangkok,  Thailand}\\*[0pt]
B.~Asavapibhop, G.~Singh, N.~Srimanobhas, N.~Suwonjandee
\vskip\cmsinstskip
\textbf{Cukurova University,  Adana,  Turkey}\\*[0pt]
A.~Adiguzel, M.N.~Bakirci\cmsAuthorMark{39}, S.~Cerci\cmsAuthorMark{40}, C.~Dozen, I.~Dumanoglu, E.~Eskut, S.~Girgis, G.~Gokbulut, E.~Gurpinar, I.~Hos, E.E.~Kangal, A.~Kayis Topaksu, G.~Onengut\cmsAuthorMark{41}, K.~Ozdemir, S.~Ozturk\cmsAuthorMark{39}, A.~Polatoz, D.~Sunar Cerci\cmsAuthorMark{40}, B.~Tali\cmsAuthorMark{40}, H.~Topakli\cmsAuthorMark{39}, M.~Vergili
\vskip\cmsinstskip
\textbf{Middle East Technical University,  Physics Department,  Ankara,  Turkey}\\*[0pt]
I.V.~Akin, B.~Bilin, S.~Bilmis, H.~Gamsizkan\cmsAuthorMark{42}, G.~Karapinar\cmsAuthorMark{43}, K.~Ocalan\cmsAuthorMark{44}, S.~Sekmen, U.E.~Surat, M.~Yalvac, M.~Zeyrek
\vskip\cmsinstskip
\textbf{Bogazici University,  Istanbul,  Turkey}\\*[0pt]
E.~G\"{u}lmez, B.~Isildak\cmsAuthorMark{45}, M.~Kaya\cmsAuthorMark{46}, O.~Kaya\cmsAuthorMark{47}
\vskip\cmsinstskip
\textbf{Istanbul Technical University,  Istanbul,  Turkey}\\*[0pt]
K.~Cankocak, F.I.~Vardarl\i
\vskip\cmsinstskip
\textbf{National Scientific Center,  Kharkov Institute of Physics and Technology,  Kharkov,  Ukraine}\\*[0pt]
L.~Levchuk, P.~Sorokin
\vskip\cmsinstskip
\textbf{University of Bristol,  Bristol,  United Kingdom}\\*[0pt]
J.J.~Brooke, E.~Clement, D.~Cussans, H.~Flacher, J.~Goldstein, M.~Grimes, G.P.~Heath, H.F.~Heath, J.~Jacob, L.~Kreczko, C.~Lucas, Z.~Meng, D.M.~Newbold\cmsAuthorMark{48}, S.~Paramesvaran, A.~Poll, S.~Senkin, V.J.~Smith, T.~Williams
\vskip\cmsinstskip
\textbf{Rutherford Appleton Laboratory,  Didcot,  United Kingdom}\\*[0pt]
K.W.~Bell, A.~Belyaev\cmsAuthorMark{49}, C.~Brew, R.M.~Brown, D.J.A.~Cockerill, J.A.~Coughlan, K.~Harder, S.~Harper, E.~Olaiya, D.~Petyt, C.H.~Shepherd-Themistocleous, A.~Thea, I.R.~Tomalin, W.J.~Womersley, S.D.~Worm
\vskip\cmsinstskip
\textbf{Imperial College,  London,  United Kingdom}\\*[0pt]
M.~Baber, R.~Bainbridge, O.~Buchmuller, D.~Burton, D.~Colling, N.~Cripps, M.~Cutajar, P.~Dauncey, G.~Davies, M.~Della Negra, P.~Dunne, W.~Ferguson, J.~Fulcher, D.~Futyan, A.~Gilbert, G.~Hall, G.~Iles, M.~Jarvis, G.~Karapostoli, M.~Kenzie, R.~Lane, R.~Lucas\cmsAuthorMark{48}, L.~Lyons, A.-M.~Magnan, S.~Malik, B.~Mathias, J.~Nash, A.~Nikitenko\cmsAuthorMark{37}, J.~Pela, M.~Pesaresi, K.~Petridis, D.M.~Raymond, S.~Rogerson, A.~Rose, C.~Seez, P.~Sharp$^{\textrm{\dag}}$, A.~Tapper, M.~Vazquez Acosta, T.~Virdee, S.C.~Zenz
\vskip\cmsinstskip
\textbf{Brunel University,  Uxbridge,  United Kingdom}\\*[0pt]
J.E.~Cole, P.R.~Hobson, A.~Khan, P.~Kyberd, D.~Leggat, D.~Leslie, W.~Martin, I.D.~Reid, P.~Symonds, L.~Teodorescu, M.~Turner
\vskip\cmsinstskip
\textbf{Baylor University,  Waco,  USA}\\*[0pt]
J.~Dittmann, K.~Hatakeyama, A.~Kasmi, H.~Liu, T.~Scarborough
\vskip\cmsinstskip
\textbf{The University of Alabama,  Tuscaloosa,  USA}\\*[0pt]
O.~Charaf, S.I.~Cooper, C.~Henderson, P.~Rumerio
\vskip\cmsinstskip
\textbf{Boston University,  Boston,  USA}\\*[0pt]
A.~Avetisyan, T.~Bose, C.~Fantasia, P.~Lawson, C.~Richardson, J.~Rohlf, J.~St.~John, L.~Sulak
\vskip\cmsinstskip
\textbf{Brown University,  Providence,  USA}\\*[0pt]
J.~Alimena, E.~Berry, S.~Bhattacharya, G.~Christopher, D.~Cutts, Z.~Demiragli, N.~Dhingra, A.~Ferapontov, A.~Garabedian, U.~Heintz, G.~Kukartsev, E.~Laird, G.~Landsberg, M.~Luk, M.~Narain, M.~Segala, T.~Sinthuprasith, T.~Speer, J.~Swanson
\vskip\cmsinstskip
\textbf{University of California,  Davis,  Davis,  USA}\\*[0pt]
R.~Breedon, G.~Breto, M.~Calderon De La Barca Sanchez, S.~Chauhan, M.~Chertok, J.~Conway, R.~Conway, P.T.~Cox, R.~Erbacher, M.~Gardner, W.~Ko, R.~Lander, T.~Miceli, M.~Mulhearn, D.~Pellett, J.~Pilot, F.~Ricci-Tam, M.~Searle, S.~Shalhout, J.~Smith, M.~Squires, D.~Stolp, M.~Tripathi, S.~Wilbur, R.~Yohay
\vskip\cmsinstskip
\textbf{University of California,  Los Angeles,  USA}\\*[0pt]
R.~Cousins, P.~Everaerts, C.~Farrell, J.~Hauser, M.~Ignatenko, G.~Rakness, E.~Takasugi, V.~Valuev, M.~Weber
\vskip\cmsinstskip
\textbf{University of California,  Riverside,  Riverside,  USA}\\*[0pt]
K.~Burt, R.~Clare, J.~Ellison, J.W.~Gary, G.~Hanson, J.~Heilman, M.~Ivova Rikova, P.~Jandir, E.~Kennedy, F.~Lacroix, O.R.~Long, A.~Luthra, M.~Malberti, H.~Nguyen, M.~Olmedo Negrete, A.~Shrinivas, S.~Sumowidagdo, S.~Wimpenny
\vskip\cmsinstskip
\textbf{University of California,  San Diego,  La Jolla,  USA}\\*[0pt]
W.~Andrews, J.G.~Branson, G.B.~Cerati, S.~Cittolin, R.T.~D'Agnolo, D.~Evans, A.~Holzner, R.~Kelley, D.~Klein, D.~Kovalskyi, M.~Lebourgeois, J.~Letts, I.~Macneill, D.~Olivito, S.~Padhi, C.~Palmer, M.~Pieri, M.~Sani, V.~Sharma, S.~Simon, E.~Sudano, Y.~Tu, A.~Vartak, C.~Welke, F.~W\"{u}rthwein, A.~Yagil
\vskip\cmsinstskip
\textbf{University of California,  Santa Barbara,  Santa Barbara,  USA}\\*[0pt]
D.~Barge, J.~Bradmiller-Feld, C.~Campagnari, T.~Danielson, A.~Dishaw, K.~Flowers, M.~Franco Sevilla, P.~Geffert, C.~George, F.~Golf, L.~Gouskos, J.~Incandela, C.~Justus, N.~Mccoll, J.~Richman, D.~Stuart, W.~To, C.~West, J.~Yoo
\vskip\cmsinstskip
\textbf{California Institute of Technology,  Pasadena,  USA}\\*[0pt]
A.~Apresyan, A.~Bornheim, J.~Bunn, Y.~Chen, J.~Duarte, A.~Mott, H.B.~Newman, C.~Pena, C.~Rogan, M.~Spiropulu, V.~Timciuc, J.R.~Vlimant, R.~Wilkinson, S.~Xie, R.Y.~Zhu
\vskip\cmsinstskip
\textbf{Carnegie Mellon University,  Pittsburgh,  USA}\\*[0pt]
V.~Azzolini, A.~Calamba, B.~Carlson, T.~Ferguson, Y.~Iiyama, M.~Paulini, J.~Russ, H.~Vogel, I.~Vorobiev
\vskip\cmsinstskip
\textbf{University of Colorado at Boulder,  Boulder,  USA}\\*[0pt]
J.P.~Cumalat, W.T.~Ford, A.~Gaz, E.~Luiggi Lopez, U.~Nauenberg, J.G.~Smith, K.~Stenson, K.A.~Ulmer, S.R.~Wagner
\vskip\cmsinstskip
\textbf{Cornell University,  Ithaca,  USA}\\*[0pt]
J.~Alexander, A.~Chatterjee, J.~Chu, S.~Dittmer, N.~Eggert, N.~Mirman, G.~Nicolas Kaufman, J.R.~Patterson, A.~Ryd, E.~Salvati, L.~Skinnari, W.~Sun, W.D.~Teo, J.~Thom, J.~Thompson, J.~Tucker, Y.~Weng, L.~Winstrom, P.~Wittich
\vskip\cmsinstskip
\textbf{Fairfield University,  Fairfield,  USA}\\*[0pt]
D.~Winn
\vskip\cmsinstskip
\textbf{Fermi National Accelerator Laboratory,  Batavia,  USA}\\*[0pt]
S.~Abdullin, M.~Albrow, J.~Anderson, G.~Apollinari, L.A.T.~Bauerdick, A.~Beretvas, J.~Berryhill, P.C.~Bhat, G.~Bolla, K.~Burkett, J.N.~Butler, H.W.K.~Cheung, F.~Chlebana, S.~Cihangir, V.D.~Elvira, I.~Fisk, J.~Freeman, Y.~Gao, E.~Gottschalk, L.~Gray, D.~Green, S.~Gr\"{u}nendahl, O.~Gutsche, J.~Hanlon, D.~Hare, R.M.~Harris, J.~Hirschauer, B.~Hooberman, S.~Jindariani, M.~Johnson, U.~Joshi, K.~Kaadze, B.~Klima, B.~Kreis, S.~Kwan, J.~Linacre, D.~Lincoln, R.~Lipton, T.~Liu, J.~Lykken, K.~Maeshima, J.M.~Marraffino, V.I.~Martinez Outschoorn, S.~Maruyama, D.~Mason, P.~McBride, P.~Merkel, K.~Mishra, S.~Mrenna, Y.~Musienko\cmsAuthorMark{29}, S.~Nahn, C.~Newman-Holmes, V.~O'Dell, O.~Prokofyev, E.~Sexton-Kennedy, S.~Sharma, A.~Soha, W.J.~Spalding, L.~Spiegel, L.~Taylor, S.~Tkaczyk, N.V.~Tran, L.~Uplegger, E.W.~Vaandering, R.~Vidal, A.~Whitbeck, J.~Whitmore, F.~Yang
\vskip\cmsinstskip
\textbf{University of Florida,  Gainesville,  USA}\\*[0pt]
D.~Acosta, P.~Avery, P.~Bortignon, D.~Bourilkov, M.~Carver, T.~Cheng, D.~Curry, S.~Das, M.~De Gruttola, G.P.~Di Giovanni, R.D.~Field, M.~Fisher, I.K.~Furic, J.~Hugon, J.~Konigsberg, A.~Korytov, T.~Kypreos, J.F.~Low, K.~Matchev, P.~Milenovic\cmsAuthorMark{50}, G.~Mitselmakher, L.~Muniz, A.~Rinkevicius, L.~Shchutska, M.~Snowball, D.~Sperka, J.~Yelton, M.~Zakaria
\vskip\cmsinstskip
\textbf{Florida International University,  Miami,  USA}\\*[0pt]
S.~Hewamanage, S.~Linn, P.~Markowitz, G.~Martinez, J.L.~Rodriguez
\vskip\cmsinstskip
\textbf{Florida State University,  Tallahassee,  USA}\\*[0pt]
T.~Adams, A.~Askew, J.~Bochenek, B.~Diamond, J.~Haas, S.~Hagopian, V.~Hagopian, K.F.~Johnson, H.~Prosper, V.~Veeraraghavan, M.~Weinberg
\vskip\cmsinstskip
\textbf{Florida Institute of Technology,  Melbourne,  USA}\\*[0pt]
M.M.~Baarmand, M.~Hohlmann, H.~Kalakhety, F.~Yumiceva
\vskip\cmsinstskip
\textbf{University of Illinois at Chicago~(UIC), ~Chicago,  USA}\\*[0pt]
M.R.~Adams, L.~Apanasevich, V.E.~Bazterra, D.~Berry, R.R.~Betts, I.~Bucinskaite, R.~Cavanaugh, O.~Evdokimov, L.~Gauthier, C.E.~Gerber, D.J.~Hofman, S.~Khalatyan, P.~Kurt, D.H.~Moon, C.~O'Brien, C.~Silkworth, P.~Turner, N.~Varelas
\vskip\cmsinstskip
\textbf{The University of Iowa,  Iowa City,  USA}\\*[0pt]
E.A.~Albayrak\cmsAuthorMark{51}, B.~Bilki\cmsAuthorMark{52}, W.~Clarida, K.~Dilsiz, F.~Duru, M.~Haytmyradov, J.-P.~Merlo, H.~Mermerkaya\cmsAuthorMark{53}, A.~Mestvirishvili, A.~Moeller, J.~Nachtman, H.~Ogul, Y.~Onel, F.~Ozok\cmsAuthorMark{51}, A.~Penzo, R.~Rahmat, S.~Sen, P.~Tan, E.~Tiras, J.~Wetzel, T.~Yetkin\cmsAuthorMark{54}, K.~Yi
\vskip\cmsinstskip
\textbf{Johns Hopkins University,  Baltimore,  USA}\\*[0pt]
B.A.~Barnett, B.~Blumenfeld, S.~Bolognesi, D.~Fehling, A.V.~Gritsan, P.~Maksimovic, C.~Martin, M.~Swartz
\vskip\cmsinstskip
\textbf{The University of Kansas,  Lawrence,  USA}\\*[0pt]
P.~Baringer, A.~Bean, G.~Benelli, C.~Bruner, R.P.~Kenny III, M.~Malek, M.~Murray, D.~Noonan, S.~Sanders, J.~Sekaric, R.~Stringer, Q.~Wang, J.S.~Wood
\vskip\cmsinstskip
\textbf{Kansas State University,  Manhattan,  USA}\\*[0pt]
A.F.~Barfuss, I.~Chakaberia, A.~Ivanov, S.~Khalil, M.~Makouski, Y.~Maravin, L.K.~Saini, S.~Shrestha, N.~Skhirtladze, I.~Svintradze
\vskip\cmsinstskip
\textbf{Lawrence Livermore National Laboratory,  Livermore,  USA}\\*[0pt]
J.~Gronberg, D.~Lange, F.~Rebassoo, D.~Wright
\vskip\cmsinstskip
\textbf{University of Maryland,  College Park,  USA}\\*[0pt]
A.~Baden, A.~Belloni, B.~Calvert, S.C.~Eno, J.A.~Gomez, N.J.~Hadley, R.G.~Kellogg, T.~Kolberg, Y.~Lu, M.~Marionneau, A.C.~Mignerey, K.~Pedro, A.~Skuja, M.B.~Tonjes, S.C.~Tonwar
\vskip\cmsinstskip
\textbf{Massachusetts Institute of Technology,  Cambridge,  USA}\\*[0pt]
A.~Apyan, R.~Barbieri, G.~Bauer, W.~Busza, I.A.~Cali, M.~Chan, L.~Di Matteo, V.~Dutta, G.~Gomez Ceballos, M.~Goncharov, D.~Gulhan, M.~Klute, Y.S.~Lai, Y.-J.~Lee, A.~Levin, P.D.~Luckey, T.~Ma, C.~Paus, D.~Ralph, C.~Roland, G.~Roland, G.S.F.~Stephans, F.~St\"{o}ckli, K.~Sumorok, D.~Velicanu, J.~Veverka, B.~Wyslouch, M.~Yang, M.~Zanetti, V.~Zhukova
\vskip\cmsinstskip
\textbf{University of Minnesota,  Minneapolis,  USA}\\*[0pt]
B.~Dahmes, A.~Gude, S.C.~Kao, K.~Klapoetke, Y.~Kubota, J.~Mans, N.~Pastika, R.~Rusack, A.~Singovsky, N.~Tambe, J.~Turkewitz
\vskip\cmsinstskip
\textbf{University of Mississippi,  Oxford,  USA}\\*[0pt]
J.G.~Acosta, S.~Oliveros
\vskip\cmsinstskip
\textbf{University of Nebraska-Lincoln,  Lincoln,  USA}\\*[0pt]
E.~Avdeeva, K.~Bloom, S.~Bose, D.R.~Claes, A.~Dominguez, R.~Gonzalez Suarez, J.~Keller, D.~Knowlton, I.~Kravchenko, J.~Lazo-Flores, S.~Malik, F.~Meier, G.R.~Snow, M.~Zvada
\vskip\cmsinstskip
\textbf{State University of New York at Buffalo,  Buffalo,  USA}\\*[0pt]
J.~Dolen, A.~Godshalk, I.~Iashvili, A.~Kharchilava, A.~Kumar, S.~Rappoccio
\vskip\cmsinstskip
\textbf{Northeastern University,  Boston,  USA}\\*[0pt]
G.~Alverson, E.~Barberis, D.~Baumgartel, M.~Chasco, J.~Haley, A.~Massironi, D.M.~Morse, D.~Nash, T.~Orimoto, D.~Trocino, R.-J.~Wang, D.~Wood, J.~Zhang
\vskip\cmsinstskip
\textbf{Northwestern University,  Evanston,  USA}\\*[0pt]
K.A.~Hahn, A.~Kubik, N.~Mucia, N.~Odell, B.~Pollack, A.~Pozdnyakov, M.~Schmitt, S.~Stoynev, K.~Sung, M.~Velasco, S.~Won
\vskip\cmsinstskip
\textbf{University of Notre Dame,  Notre Dame,  USA}\\*[0pt]
A.~Brinkerhoff, K.M.~Chan, A.~Drozdetskiy, M.~Hildreth, C.~Jessop, D.J.~Karmgard, N.~Kellams, K.~Lannon, W.~Luo, S.~Lynch, N.~Marinelli, T.~Pearson, M.~Planer, R.~Ruchti, N.~Valls, M.~Wayne, M.~Wolf, A.~Woodard
\vskip\cmsinstskip
\textbf{The Ohio State University,  Columbus,  USA}\\*[0pt]
L.~Antonelli, J.~Brinson, B.~Bylsma, L.S.~Durkin, S.~Flowers, A.~Hart, C.~Hill, R.~Hughes, K.~Kotov, T.Y.~Ling, D.~Puigh, M.~Rodenburg, G.~Smith, B.L.~Winer, H.~Wolfe, H.W.~Wulsin
\vskip\cmsinstskip
\textbf{Princeton University,  Princeton,  USA}\\*[0pt]
O.~Driga, P.~Elmer, P.~Hebda, A.~Hunt, S.A.~Koay, P.~Lujan, D.~Marlow, T.~Medvedeva, M.~Mooney, J.~Olsen, P.~Pirou\'{e}, X.~Quan, H.~Saka, D.~Stickland\cmsAuthorMark{2}, C.~Tully, J.S.~Werner, A.~Zuranski
\vskip\cmsinstskip
\textbf{University of Puerto Rico,  Mayaguez,  USA}\\*[0pt]
E.~Brownson, H.~Mendez, J.E.~Ramirez Vargas
\vskip\cmsinstskip
\textbf{Purdue University,  West Lafayette,  USA}\\*[0pt]
V.E.~Barnes, D.~Benedetti, D.~Bortoletto, M.~De Mattia, L.~Gutay, Z.~Hu, M.K.~Jha, M.~Jones, K.~Jung, M.~Kress, N.~Leonardo, D.~Lopes Pegna, V.~Maroussov, D.H.~Miller, N.~Neumeister, B.C.~Radburn-Smith, X.~Shi, I.~Shipsey, D.~Silvers, A.~Svyatkovskiy, F.~Wang, W.~Xie, L.~Xu, H.D.~Yoo, J.~Zablocki, Y.~Zheng
\vskip\cmsinstskip
\textbf{Purdue University Calumet,  Hammond,  USA}\\*[0pt]
N.~Parashar, J.~Stupak
\vskip\cmsinstskip
\textbf{Rice University,  Houston,  USA}\\*[0pt]
A.~Adair, B.~Akgun, K.M.~Ecklund, F.J.M.~Geurts, W.~Li, B.~Michlin, B.P.~Padley, R.~Redjimi, J.~Roberts, J.~Zabel
\vskip\cmsinstskip
\textbf{University of Rochester,  Rochester,  USA}\\*[0pt]
B.~Betchart, A.~Bodek, R.~Covarelli, P.~de Barbaro, R.~Demina, Y.~Eshaq, T.~Ferbel, A.~Garcia-Bellido, P.~Goldenzweig, J.~Han, A.~Harel, A.~Khukhunaishvili, G.~Petrillo, D.~Vishnevskiy
\vskip\cmsinstskip
\textbf{The Rockefeller University,  New York,  USA}\\*[0pt]
R.~Ciesielski, L.~Demortier, K.~Goulianos, G.~Lungu, C.~Mesropian
\vskip\cmsinstskip
\textbf{Rutgers,  The State University of New Jersey,  Piscataway,  USA}\\*[0pt]
S.~Arora, A.~Barker, J.P.~Chou, C.~Contreras-Campana, E.~Contreras-Campana, D.~Duggan, D.~Ferencek, Y.~Gershtein, R.~Gray, E.~Halkiadakis, D.~Hidas, S.~Kaplan, A.~Lath, S.~Panwalkar, M.~Park, R.~Patel, S.~Salur, S.~Schnetzer, S.~Somalwar, R.~Stone, S.~Thomas, P.~Thomassen, M.~Walker
\vskip\cmsinstskip
\textbf{University of Tennessee,  Knoxville,  USA}\\*[0pt]
K.~Rose, S.~Spanier, A.~York
\vskip\cmsinstskip
\textbf{Texas A\&M University,  College Station,  USA}\\*[0pt]
O.~Bouhali\cmsAuthorMark{55}, A.~Castaneda Hernandez, R.~Eusebi, W.~Flanagan, J.~Gilmore, T.~Kamon\cmsAuthorMark{56}, V.~Khotilovich, V.~Krutelyov, R.~Montalvo, I.~Osipenkov, Y.~Pakhotin, A.~Perloff, J.~Roe, A.~Rose, A.~Safonov, T.~Sakuma, I.~Suarez, A.~Tatarinov
\vskip\cmsinstskip
\textbf{Texas Tech University,  Lubbock,  USA}\\*[0pt]
N.~Akchurin, C.~Cowden, J.~Damgov, C.~Dragoiu, P.R.~Dudero, J.~Faulkner, K.~Kovitanggoon, S.~Kunori, S.W.~Lee, T.~Libeiro, I.~Volobouev
\vskip\cmsinstskip
\textbf{Vanderbilt University,  Nashville,  USA}\\*[0pt]
E.~Appelt, A.G.~Delannoy, S.~Greene, A.~Gurrola, W.~Johns, C.~Maguire, Y.~Mao, A.~Melo, M.~Sharma, P.~Sheldon, B.~Snook, S.~Tuo, J.~Velkovska
\vskip\cmsinstskip
\textbf{University of Virginia,  Charlottesville,  USA}\\*[0pt]
M.W.~Arenton, S.~Boutle, B.~Cox, B.~Francis, J.~Goodell, R.~Hirosky, A.~Ledovskoy, H.~Li, C.~Lin, C.~Neu, J.~Wood
\vskip\cmsinstskip
\textbf{Wayne State University,  Detroit,  USA}\\*[0pt]
C.~Clarke, R.~Harr, P.E.~Karchin, C.~Kottachchi Kankanamge Don, P.~Lamichhane, J.~Sturdy
\vskip\cmsinstskip
\textbf{University of Wisconsin,  Madison,  USA}\\*[0pt]
D.A.~Belknap, D.~Carlsmith, M.~Cepeda, S.~Dasu, L.~Dodd, S.~Duric, E.~Friis, R.~Hall-Wilton, M.~Herndon, A.~Herv\'{e}, P.~Klabbers, A.~Lanaro, C.~Lazaridis, A.~Levine, R.~Loveless, A.~Mohapatra, I.~Ojalvo, T.~Perry, G.A.~Pierro, G.~Polese, I.~Ross, T.~Sarangi, A.~Savin, W.H.~Smith, D.~Taylor, P.~Verwilligen, C.~Vuosalo, N.~Woods
\vskip\cmsinstskip
\dag:~Deceased\\
1:~~Also at Vienna University of Technology, Vienna, Austria\\
2:~~Also at CERN, European Organization for Nuclear Research, Geneva, Switzerland\\
3:~~Also at Institut Pluridisciplinaire Hubert Curien, Universit\'{e}~de Strasbourg, Universit\'{e}~de Haute Alsace Mulhouse, CNRS/IN2P3, Strasbourg, France\\
4:~~Also at National Institute of Chemical Physics and Biophysics, Tallinn, Estonia\\
5:~~Also at Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Moscow, Russia\\
6:~~Also at Universidade Estadual de Campinas, Campinas, Brazil\\
7:~~Also at Laboratoire Leprince-Ringuet, Ecole Polytechnique, IN2P3-CNRS, Palaiseau, France\\
8:~~Also at Joint Institute for Nuclear Research, Dubna, Russia\\
9:~~Also at Suez University, Suez, Egypt\\
10:~Also at Cairo University, Cairo, Egypt\\
11:~Also at Fayoum University, El-Fayoum, Egypt\\
12:~Also at British University in Egypt, Cairo, Egypt\\
13:~Now at Sultan Qaboos University, Muscat, Oman\\
14:~Also at Universit\'{e}~de Haute Alsace, Mulhouse, France\\
15:~Also at Brandenburg University of Technology, Cottbus, Germany\\
16:~Also at Institute of Nuclear Research ATOMKI, Debrecen, Hungary\\
17:~Also at E\"{o}tv\"{o}s Lor\'{a}nd University, Budapest, Hungary\\
18:~Also at University of Debrecen, Debrecen, Hungary\\
19:~Also at University of Visva-Bharati, Santiniketan, India\\
20:~Now at King Abdulaziz University, Jeddah, Saudi Arabia\\
21:~Also at University of Ruhuna, Matara, Sri Lanka\\
22:~Also at Isfahan University of Technology, Isfahan, Iran\\
23:~Also at Sharif University of Technology, Tehran, Iran\\
24:~Also at Plasma Physics Research Center, Science and Research Branch, Islamic Azad University, Tehran, Iran\\
25:~Also at Universit\`{a}~degli Studi di Siena, Siena, Italy\\
26:~Also at Centre National de la Recherche Scientifique~(CNRS)~-~IN2P3, Paris, France\\
27:~Also at Purdue University, West Lafayette, USA\\
28:~Also at Universidad Michoacana de San Nicolas de Hidalgo, Morelia, Mexico\\
29:~Also at Institute for Nuclear Research, Moscow, Russia\\
30:~Also at St.~Petersburg State Polytechnical University, St.~Petersburg, Russia\\
31:~Also at California Institute of Technology, Pasadena, USA\\
32:~Also at Faculty of Physics, University of Belgrade, Belgrade, Serbia\\
33:~Also at Facolt\`{a}~Ingegneria, Universit\`{a}~di Roma, Roma, Italy\\
34:~Also at Scuola Normale e~Sezione dell'INFN, Pisa, Italy\\
35:~Also at University of Athens, Athens, Greece\\
36:~Also at Paul Scherrer Institut, Villigen, Switzerland\\
37:~Also at Institute for Theoretical and Experimental Physics, Moscow, Russia\\
38:~Also at Albert Einstein Center for Fundamental Physics, Bern, Switzerland\\
39:~Also at Gaziosmanpasa University, Tokat, Turkey\\
40:~Also at Adiyaman University, Adiyaman, Turkey\\
41:~Also at Cag University, Mersin, Turkey\\
42:~Also at Anadolu University, Eskisehir, Turkey\\
43:~Also at Izmir Institute of Technology, Izmir, Turkey\\
44:~Also at Necmettin Erbakan University, Konya, Turkey\\
45:~Also at Ozyegin University, Istanbul, Turkey\\
46:~Also at Marmara University, Istanbul, Turkey\\
47:~Also at Kafkas University, Kars, Turkey\\
48:~Also at Rutherford Appleton Laboratory, Didcot, United Kingdom\\
49:~Also at School of Physics and Astronomy, University of Southampton, Southampton, United Kingdom\\
50:~Also at University of Belgrade, Faculty of Physics and Vinca Institute of Nuclear Sciences, Belgrade, Serbia\\
51:~Also at Mimar Sinan University, Istanbul, Istanbul, Turkey\\
52:~Also at Argonne National Laboratory, Argonne, USA\\
53:~Also at Erzincan University, Erzincan, Turkey\\
54:~Also at Yildiz Technical University, Istanbul, Turkey\\
55:~Also at Texas A\&M University at Qatar, Doha, Qatar\\
56:~Also at Kyungpook National University, Daegu, Korea\\


